Data-driven analysis of central bank digital currency (CBDC) projects drivers

In this paper, we use a variety of machine learning methods to quantify the extent to which economic and technological factors are predictive of the progression of Central Bank Digital Currencies (CBDC) within a country, using as our measure of this progression the CBDC project index (CBDCPI). We find that a financial development index is the most important feature for our model, followed by the GDP per capita and an index of the voice and accountability of the country's population. Our results are consistent with previous qualitative research which finds that countries with a high degree of financial development or digital infrastructure have more developed CBDC projects. Further, we obtain robust results when predicting the CBDCPI at different points in time.

==> sections/5-future_work.tex <==
\section{Future Work}

Features of the CME Bitcoin futures contract, combined with the relative nascency of the financial product, resulted in a small sample size. Therefore, it is likely that evidence of market inefficiency would not have been detected even if it did exist. Thus future work can apply the methodology proposed to larger data sets when they become available, or to try with other Bitcoin future markets data. For example, Kraken offers several futures contract pairs, including BTC/USD, ETH/USD, LTCUSD,	BCH/USD, XRP/USD and XRP/BTC. Also, OKEx and BitMEX, although they are unregulated marketplaces, each have average daily volumes exceeding \$1 billion, making them the two largest bitcoin futures exchanges available today. Testing with data from these markets would ensure robustness of the empirical results.

Additionally, larger data sets would enable us introduce autoregressive moving average (ARMA) model\footnote{ARMA models provide a description of a weak stationary stochastic process in terms of two processes: Autoregression (AR($p$)) model and Moving average (MA($q$)) model. The model is usually referred to as ARMA($p,q$) model where $p$ is the number of AR terms and $q$ is the number of MA terms. The AR part denotes regressing the variable on its own lagged (i.e., past) series values. The MA part models the error term as a linear combination of residual terms of various times in the past.}, as tested in \cite{CANARELLA1986575,Otto2011}. The ARMA approach is one of the promising ways to empirically test the speculative efficiency hypothesis with overlapping data sets, which avoid reducing the sample size and loss of information. We omitted this method as from the econometric point of view, the rule of thumb is that at least 50, but ideally more than 100 observations, should be estimated for ARMA models \cite{Box1975} and our samples doesn't meet this criteria. For the CME Bitcoin futures overlapping price to be analyzed with ARMA, we need to wait for enough data to be accumulated, unless new types of commodities emerges.

